Predicting Attention Sparsity in Transformers

Transformers' quadratic complexity with respect to the input sequence length has motivated a body of work on efficient sparse approximations to softmax. An alternative path, used by entmax transformers, consists of having built-in exact sparse attention; however this approach still requires quadratic computation. In this paper, we propose Sparsefinder, a simple model trained to identify the sparsity pattern of entmax attention before computing it. We experiment with three variants of our method, based on distances, quantization, and clustering, on two tasks: machine translation (attention in the decoder) and masked language modeling (encoder-only). Our work provides a new angle to study model efficiency by doing extensive analysis of the tradeoff between the sparsity and recall of the predicted attention graph. This allows for detailed comparison between different models along their Pareto curves, important to guide future benchmarks for sparse attention models.

==> table_document_level_results.tex <==
\begin{table*}[t]
    \small
    \begin{center}
    \begin{tabular}{l@{  }l ccccc@{ }c ccccc@{ }c}
        \toprule
         & & \multicolumn{5}{c}{\sc IWSLT17 (en$\to$de)} & & \multicolumn{5}{c}{\sc IWSLT17 (en$\to$fr)} \\
        \cmidrule{3-7} \cmidrule{9-13}
        \sc Model & & $S$ & $R$ & BLEU & COMET & \textsc{Cont.} & & $S$ & $R$ & BLEU & COMET & \textsc{Cont.} \\
        \midrule 
 
        
        Transformer     & & 79.94 & 100.0 & 34.72 & 0.5194 & 0.6622        & & 0.84 & 1.00 & 43.49 & 0.68 & 0.81 \\
        Sf. distance    & & 55.06 & 85.44 & 34.56 & 0.5139 & 0.6705      & & 0.58 & 0.73 & 43.43 & 0.67 & 0.78 \\
        Sf. quant.      & & 50.36 & 80.18 & 34.87 & 0.5188 & 0.5744      & & 0.58 & 0.73 & 43.43 & 0.67 & 0.78 \\
        Sf. k-means     & & 57.90 & 76.43 & 34.93 & 0.5184 & 0.5755      & & 0.33 & 0.88 & 43.19 & 0.66 & 0.77 \\
       
       
        \bottomrule
    \end{tabular}
    \end{center}
    \caption{Document-level MT results with 2 target context sentences and window size set to 2. $S$ and $R$ indicate sparsity and recall, respectively. \textsc{Cont.} represents the accuracy obtained on the contrastive dataset of each language pair.} 
    \label{table:results_document_nmt}
\end{table*}




       


==> table_glue.tex <==




\begin{table*}[t]
    \small
    \begin{center}
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{l@{  }l ccc@{  }c ccc@{  }c ccc@{  }c ccc@{  }c ccc}
        \toprule
        \  & &  
        \multicolumn{3}{c}{\sc MNLI} & & 
        \multicolumn{3}{c}{\sc QNLI} & & 
        \multicolumn{3}{c}{\sc MRPC} & & 
        \multicolumn{3}{c}{\sc QQP} & & 
        \multicolumn{3}{c}{\sc SQuAD1.0} \\

        \cmidrule{3-5} \cmidrule{7-9} \cmidrule{11-13} \cmidrule{15-17} \cmidrule{19-21}
        \sc Model & & $S$ & $R$ & \sc Acc & & 
                      $S$ & $R$ & \sc Acc & & 
                      $S$ & $R$ & \sc Acc & & 
                      $S$ & $R$ & \sc Acc & & 
                      $S$ & $R$ & \sc $F_1$ \\

        \midrule 
        Transformer     & & 79.50 & 100.0 & 87.00  & & 84.75 & 100.0 & 91.85  & & 81.88 & 100.0 & 85.05  & & 70.95 & 100.0 & 90.51   & & 95.74 & 100.0 & 89.11 \\
        
        
        Sf. distance    & & 46.08 & 81.97 & 85.56  & & 49.52 & 76.31 & 89.47  & & 53.20 & 83.20 & 72.06  & & 48.70& 82.21 & 89.91   & & 63.78 & 90.03 & 87.39 \\
        
        Sf. quant.      & & 28.96 & 87.73 & 86.77  & & 39.31 & 81.09 & 91.51  & & 41.76 & 79.69 & 82.84  & & 23.47 & 87.29 & 90.29   & & 63.68 & 77.94 & 84.12 \\
        
        Sf. $k$-means   & & 47.39 & 79.30 & 84.40  & & 54.69 & 72.14 & 87.97  & & 57.95 & 74.64 & 70.34  & & 49.91 & 74.86 & 89.16   & & 60.34   & 82.70 & 86.14 \\
        \bottomrule
    \end{tabular}
    } %
    \end{center}
    \caption{Results on GLUE benchmark.} 
    \label{table:results_glue}
\end{table*}

==> table_lm_roberta.tex <==
\begin{table}[!htb]
    \small
    \begin{center}
    \begin{tabular}{lcc}
        \toprule
        \sc Model & \sc Window size & \sc Perpl. \\
        \midrule
        Transformer     &  1    & 0.00 \\
        BigBird         &  1    & 0.00 \\
        Longformer      &  1    & 0.00 \\
        Reformer        &  1    & 0.00 \\
        Routing         &  1    & 0.00 \\
        Sparsefinder    &  1    & 0.00 \\
        \midrule
        Transformer     &  51    & 0.00 \\
        BigBird         &  51    & 0.00 \\
        Longformer      &  51    & 0.00 \\
        Reformer        &  51    & 0.00 \\
        Routing         &  51    & 0.00 \\
        Sparsefinder    &  51    & 0.00 \\
        \midrule
        Transformer     &  101    & 0.00 \\
        BigBird         &  101    & 0.00 \\
        Longformer      &  101    & 0.00 \\
        Reformer        &  101    & 0.00 \\
        Routing         &  101    & 0.00 \\
        Sparsefinder    &  101    & 0.00 \\
        \midrule
        Transformer     &  151    & 0.00 \\
        BigBird         &  151    & 0.00 \\
        Longformer      &  151    & 0.00 \\
        Reformer        &  151    & 0.00 \\
        Routing         &  151    & 0.00 \\
        Sparsefinder    &  151    & 0.00 \\
        \midrule
        Transformer     &  201    & 0.00 \\
        BigBird         &  201    & 0.00 \\
        Longformer      &  201    & 0.00 \\
        Reformer        &  201    & 0.00 \\
        Routing         &  201    & 0.00 \\
        Sparsefinder    &  201    & 0.00 \\
        \bottomrule
    \end{tabular}
    \end{center}
    \caption{Results on Wikitext 103 by varying window size.}
    \label{table:results_lm_roberta}
\end{table}


==> table_sentence_level_extrapolation.tex <==
\begin{table*}[t]
    \small
    \begin{center}
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{l@{  }l cccc@{ }c cccc@{ }c cccc@{ }c}
        \toprule
         & & \multicolumn{4}{c}{\sc IWSLT17 (en$\to$de)} & & \multicolumn{4}{c}{\sc OpenSubs (en$\to$fr)} & & \multicolumn{4}{c}{\sc Chat (en$\to$de)} \\
        \cmidrule{3-6} \cmidrule{8-11} \cmidrule{13-16}
        \sc Model & & $S$ & $R$ & BLEU & COMET && $S$ & $R$ & BLEU & COMET && $S$ & $R$ & BLEU & COMET \\
        \midrule 
        Transformer Base	    & & 0.41   & 0.70 & 69.41   & 70.07   	& & 0.30   & 0.67 & 67.30   & 66.67   	& & 0.38   & 0.91 & 92.38   & 91.14 \\
        Extender [10-20]  	    & & 0.41   & 0.70 & 69.41   & 70.07   	& & 0.30   & 0.67 & 67.30   & 66.67   	& & 0.38   & 0.91 & 92.38   & 91.14 \\
        Extender [20-30]  	    & & 0.41   & 0.70 & 69.41   & 70.07   	& & 0.30   & 0.67 & 67.30   & 66.67   	& & 0.38   & 0.91 & 92.38   & 91.14 \\
        Extender [30-40]  	    & & 0.41   & 0.70 & 69.41   & 70.07   	& & 0.30   & 0.67 & 67.30   & 66.67   	& & 0.38   & 0.91 & 92.38   & 91.14 \\
        Extender [30-$\infty$]  	& & 0.41   & 0.70 & 69.41   & 70.07   	& & 0.30   & 0.67 & 67.30   & 66.67   	& & 0.38   & 0.91 & 92.38   & 91.14 \\
        Extender [40-$\infty$]  	& & 0.41   & 0.70 & 69.41   & 70.07   	& & 0.30   & 0.67 & 67.30   & 66.67   	& & 0.38   & 0.91 & 92.38   & 91.14 \\
        \bottomrule
    \end{tabular}
    } %
    \end{center}
    \caption{Extrapolation results for sentence-level MT. $S$ and $R$ represent averaged sparsity and recall of all attention heads across all layers (with std numbers in parenthesis), respectively.} 
    \label{table:results_extrapolation_nmt}
\end{table*}

